Teaching Intuitionistic and Classical Propositional Logic Using Isabelle

We describe a natural deduction formalization of intuitionistic and classical propositional logic in the Isabelle/Pure framework. In contrast to earlier work, where we explored the pedagogical benefits of using a deep embedding approach to logical modelling, here we employ a logical framework modelling. This gives rise to simple and natural teaching examples and we report on the role it played in teaching our Automated Reasoning course in 2020 and 2021.

==> eptcsdata.tex <==
\providecommand{\firstpage}{71}
\providecommand{\publicationstatus}{J. Marcos, W. Neuper and P. Quaresma (Eds.): Theorem Proving Components\\ for Educational Software 2021 (ThEdu'21)\\
EPTCS 354, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.354.6}{10.4204/EPTCS.354.6}}
\pdfoutput=1

